Two Tales of Persona in LLMs: A Survey of Role-Playing and Personalization

The concept of persona, originally adopted in dialogue literature, has re-surged as a promising framework for tailoring large language models (LLMs) to specific context (e.g., personalized search, LLM-as-a-judge). However, the growing research on leveraging persona in LLMs is relatively disorganized and lacks a systematic taxonomy. To close the gap, we present a comprehensive survey to categorize the current state of the field. We identify two lines of research, namely (1) LLM Role-Playing, where personas are assigned to LLMs, and (2) LLM Personalization, where LLMs take care of user personas. Additionally, we introduce existing methods for LLM personality evaluation. To the best of our knowledge, we present the first survey for role-playing and personalization in LLMs under the unified view of persona. We continuously maintain a paper collection to foster future endeavors: https://github.com/MiuLab/PersonaLLM-Survey

==> latex/survey_struc.tex <==
\definecolor{tnodeColor}{HTML}{FFF0C5}
\definecolor{tnodeColor4}{HTML}{D9E8F6}
\definecolor{edgeColor}{HTML}{000000}
\definecolor{textColor}{HTML}{000000}

\begin{figure*}[htp!]

\centering
\resizebox{0.86\textwidth}{!}{%
\begin{forest}
  for tree={
    forked edges,
    draw=edgeColor,
    thick,
    font=\sffamily,
    fill=tnodeColor, 
    rectangle,
    rounded corners=4pt,
    text=textColor,
    blur shadow={shadow scale=0.95, shadow xshift=.5ex, shadow yshift=-.5ex, shadow opacity=0.25},
    edge={-, draw=edgeColor, line width=2pt}, 
    grow=0,
    child anchor=west,
    parent anchor=east,
    anchor=west,
    align=center,
    l sep+=0.3cm,
    s sep+=0.1cm,
  },
  root/.style=  {fill=Gray!15, font=\bfseries\huge, rounded corners=6pt, text width=4cm, /tikz/align=center, inner sep=6pt},
  tnode2_1/.style={fill=Gray!15, font=\bfseries\huge, text width=12cm, /tikz/align=center, inner sep=6pt},
  tnode2_2/.style={fill=Gray!15, font=\bfseries\huge, text width=11cm, /tikz/align=center, inner sep=6pt},
  tnode2_3/.style={fill=Gray!15, font=\bfseries\huge, text width=12cm, /tikz/align=center, inner sep=6pt},
  tnode3_1/.style={fill=Gray!15, font=\bfseries\huge, text width=12cm, /tikz/align=center, inner sep=6pt},
  tnode3_2/.style={fill=Gray!15, font=\bfseries\huge, text width=11cm, /tikz/align=center, inner sep=6pt},
  tnode3_3/.style={fill=Gray!15, font=\bfseries\huge, text width=12cm, /tikz/align=center, inner sep=6pt},
  [Taxonomy, root
    [LLM Personality Evaluation~\Cref{sec:personality}, tnode2_1
        [BigFive; MBTI; etc, tnode2_2]
    ]
    [LLM Personalization~\Cref{sec:personalized}, tnode2_1
        [Dialogue~\Cref{subsub:3-diag}, tnode2_2
            [User Persona Modeling, tnode2_3]
            [Task-Oriented Modeling, tnode2_3]
        ]
        [Healthcare~\Cref{subsub:3-healthcare}, tnode2_2]
        [Education~\Cref{subsub:3-education}, tnode2_2]
        [Search~\Cref{subsub:3-search}, tnode2_2]
        [Recommendation~\Cref{subsub:3-rec}, tnode2_2]
    ]
    [LLM Role-Playing~\Cref{sec:role_play}, tnode3_1
        [Emergent Behaviors~\Cref{subsec:2-emergent}, tnode3_2
            [Destructive Behavior, tnode3_3]
            [Conformity Behavior, tnode3_3]
            [Voluntary Behavior, tnode3_3]
        ]
        [Role-Playing Schema~\Cref{subsec:2-schema}, tnode3_2
            [Multi-Agent, tnode3_3]
            [Single-Agent, tnode3_3]
        ]
        [Environments~\Cref{subsec:2-env}, tnode3_2
            [LLM-as-Evaluator~\Cref{subsub:2-evaluator}, tnode3_3]
            [Medical Application~\Cref{subsub:2-medical}, tnode3_3]
            [Game~\Cref{subsub:2-games}, tnode3_3]
            [Software Development~\Cref{subsub:2-software}, tnode3_3]
        ]
    ]
  ]
\end{forest}
}

\caption{The taxonomy of LLM role-playing and LLM personalization.}
\label{fig:survey-struc}
% \vspace{-0.25cm}
\end{figure*}
